How to Generate Popular Post Headlines on Social Media?

Posts, as important containers of user-generated-content pieces on social media, are of tremendous social influence and commercial value. As an integral components of a post, the headline has a decisive contribution to the post's popularity. However, current mainstream method for headline generation is still manually writing, which is unstable and requires extensive human effort. This drives us to explore a novel research question: Can we automate the generation of popular headlines on social media? We collect more than 1 million posts of 42,447 celebrities from public data of Xiaohongshu, which is a well-known social media platform in China. We then conduct careful observations on the headlines of these posts. Observation results demonstrate that trends and personal styles are widespread in headlines on social medias and have significant contribution to posts's popularity. Motivated by these insights, we present MEBART, which combines Multiple preference-Extractors with Bidirectional and Auto-Regressive Transformers (BART), capturing trends and personal styles to generate popular headlines on social medias. We perform extensive experiments on real-world datasets and achieve state-of-the-art performance compared with several advanced baselines. In addition, ablation and case studies demonstrate that MEBART advances in capturing trends and personal styles.

==> djdong.tex <==
\section{observation}

\begin{figure*}[!t]
\centering
\includegraphics[width=1.0\linewidth]{analysis.pdf}
\caption{todo todo}
\label{fig:analysis}
\end{figure*}

% 最后检查！！！！！！！！！！！！！
\fzd{finally, check out these words: title\&headline, user\&author, audience, article\&post}
% 在这个章节中，我们将会对社交媒体数据集进行两个角度的分析。
In this section, we will provide an in-depth analysis of User Generated Content (UGC) platform data from two perspectives, style and trend.
% 首先，我们将会探讨在UGC平台上，用户个人发布的post的标题是否具有个人风格，并且用户是否会随着当下热点的不断变化，去影响自己post标题里面不同词语的运用。
First, we will explore whether the titles of individual user posts have a personal style and whether the user will influence the use of different words inside their post title according to the changing hot topics of the moment.
% 接下来，我们会分别分析个人风格以及紧跟潮流对文章流行度的影响。
Next, we will separately analyze the impact of personal style and keeping up with trends on the popularity of posts.
% todo
Finally, we will use a simple model to further analyze it todo.

\subsection{Dataset Descriptions}
% 介绍我们的数据
% 介绍 数据处理部分
% (1) 使用了2021年全年的数据 
% (2) 为了避免太多无意义的post的影响，我们只选取具有一定流行度的post(点赞量大于10)
% (3) 为了统计数据不受用户发布post的数量影响，我们选取每个用户发布时间最新的20篇post 

\subsection{Trend Analysis in Headlines}
% 【废案】：社交媒体上的热门话题千变万化。并且这种热门话题会吸引大量的受众追随，从而带来巨大的流量。作为想获得更多关注的社交媒体用户，他就需要紧跟潮流，去更改自己的推文主题。而文章的标题是最显眼信息，所以它可以在第一时间向受众们传达自己文章内容的主题。Hot topics on social media are ever-changing, varying from month to month, and perhaps even from day to day. And this hot topic will attract a large audience to follow, which will bring huge traffic. As a social media user who wants to get more attention, he would need to keep up with the trend and go for changing his post topics. The headline of the post are the most prominent information, so it can be the first time to convey to the audience the topic of their post content.
% 【废案】：在社交媒体上，用户既是热门话题的制造者，同时也是传播者。作为热门话题的制造者，他产出的内容一定不是一成不变的，而应该灵敏的捕捉可能成为热门的话题。
% https://www.techtarget.com/whatis/feature/9-social-media-trends
% https://influencermarketinghub.com/social-media-trends/
% https://www.themarketingeye.com/blog/hot-topics-social-media-marketing-right-now/
% Information on social media platforms is ever-changing, generating lots of hot topics every day. \hxw{As users on social media platforms, we are instinctively drawn to the hot topics of the moment.} \hxw{influenced by these popular topics, we follow the trend to change the topic of our chat or post.} The headline, as a summary of the content of the post, best reflects the topic discussed in the post. \hxw{This is not a sufficient reason to investigate trends of headlines.} So, the first research question is: \textbf{On social media, are users' post headlines influenced by trends? (Q1)}
% ----------Question one----------
\label{Q1}
% 有热门话题->热门话题变化->社交媒体上的用户follow->标题随着时间变化
% 在Google trends上，他展示了互联网上每一天都会出现大量新的热搜词语。通常来说，这些热搜词语反映了一段时间内的各界大事与流行话题,它的特点是随着时间变化，并且可以吸引大量的受众关注。通过观察小红书的数据，我们发现社交媒体平台上的用户也会跟随这些热门话题，而改变自己的文章的主题。而标题作为一个文章内容的总结提炼，最能反映出这篇文章所讨论的主题。为了仔细的研究这个现象，我们定义了问题1
On Google Trends\footnote{\url{https://trends.google.com/trends/}}, it shows that a large number of new hot searched words appear on the Internet every day. Generally speaking, these hot searched words reflect the events and popular topics of the world over a period of time. The characteristic of buzzwords is that they change over time and can attract the concern of a large audience. By observing the data of LittleRedBook, we found that users on social media platforms also follow these popular topics and change the topics of their posts. And the headline, as a summary of the content of the post, best reflects the topic discussed in this post. To scrutinize this phenomenon, we defined the first research question: \textbf{On social media, are users' post headlines influenced by trends? (Q1)}


% 分布受影响
It also means comparing whether the \hxw{distribution of} headlines has \hxw{keeping} changed  between \hxw{across?} time periods.


\hxw{update a new revision}
% So, we contrast the differences in the degree of text similarity between title pairs that are published during the same season and those that are published during separate seasons.
% 我们采样10万个标题对，这里的每个标题对里面的两个标题来自于同一季节，并计算这10万标题对的平均文本相似度。相同，我们也会采样并计算标题来自于不同季节的10万个标题对的平均文本相似度。
% We sample 100,000 title pairs, where two titles inside each title pair are from the same season, and calculate the averaged text similarity of these 100,000 title pairs. Similarly, we also sample and calculate the averaged text similarity of 100,000 title pairs whose titles come from different seasons.

For simplicity, here we use \textit{words overlap} as a measure of text similarity.
We introduce the \textit{words overlap} ($WO \in [0,1]$):
\begin{equation}
    WO(h_i, h_j) = \frac{\textit{CNT} (set(h_j) \cap set(h_j))}{\textit{CNT} (set(h_i) \cup set(h_j)},
\end{equation}
where $h_i$ and $h_j$ are the two headlines for which the text similarity is to be calculated, $set()$ is the set operation, $\textit{CNT}()$ is a counter that counts the number of words in a set. The higher the $WO$, the more similar the two texts are.

% 同时，我们为了简单对比爆文的标题随着不同季节变化的趋势，我们把这四个统计结果展示到图1a中。
% 解释图表
% 分析图表
% 通过上面的观察，我们可以发现 相比不同季度，同季度之间的标题会有更高的words overlap
% 所以我们可以的到第一个问题的结论：随着潮流的不同变化，用户的用词会有变化，并且用户的文章标题也会发生变化。
% Next，同时我们对比爆文和正常文章的words overlap，可以发现爆文的这种变化趋势要更明显，也就是对潮流更敏感。
% 从上面我们可以了解到文章的标题确实会受到潮流的影响而变化，并且爆文会对潮流的变化更敏感。

% -----Question two-----
% 直觉上，用户可能会更喜欢和当下潮流符合的文章。
Therefore, in order to investigate more deeply the relationship between such trend-following headlines on post popularity, we introduce the second question: \textbf{What effect does the trendiness of the title have on the popularity of the post? (Q2)}

% 我们把trend具体化为潮流词，也就是其他时间很少出现，只集中出现在一段时间。
% 热词并不是以前没有出现过，只是以前出现的次数比较少。
% 首先我们定义了热门词语
% 我们定义了四组，我们发现只有使用当季热词会有更高的likes
% 给出发现和结论，并且给出解释
% 我们最后的结论 不能乱用热词，要用当季的热词
% 每种现象要有对应的解释

% 为了保证对比是公平的

% 我们不知道这些热门词对标题的影响

\subsection{Personal Style Analysis in Headlines}
% ----------Question three----------
% [废案]一般来说，post的标题都是这个post内容的一个简短的总结，能让受众最快的了解到这篇post主要的表达内容，吸引受众来浏览和点赞等操作。根据观察，对于某些作者，他个人的post的标题之间可能有某种关系。具体来说，某些作者的不同post标题之间的排版格式是相似的，或者语义是相似的。这种一个作者标题之间的相似性我们称为个人风格。
% Generally speaking, the title of a post is a short summary of the content of the post, which enables the audience to understand the main content of the post and attracts them to browse and like it. It is observed that for some authors, there may be some kind of relationship between the titles of their individual posts. Specifically, the typographic formatting is similar or the semantics are similar between different post titles of certain authors. This similarity between an author's titles is what we call personal style. So, the third research question is: \textbf{Do users' post titles have a personal style on UGC platform? (Q3)}
% Social media is an essential part of people's lives nowadays, and people from different regions, genders and ages are posting their daily lives on social media. \hxw{this sentence should connect with last subsection} \hxw{On social media, posts are published by a specific user.} 
% \hxw{Intuitively,} Since different kinds of people have different language habits, thinking styles and interests.  This variability may lead to different language styles for different users, and it is even possible that users may have different styles of posting on social media. \hxw{Grammatical errors: Since A, B, which may lead C}
% \hxw{characteristic of data/application -> phenomenon -> intuition-> observation (maybe driven by problem, maybe directly observate)}
% ----- ----- ----- -----
We verified above that the headlines of posts on social media change over time, so what other factors influence the headlines? Generally, on social media, posts are published by a specific user. We observed a large number of post headlines on social media, which were published by users from different regions, genders, and ages, and we found that the post headlines of different kinds of users had very different personal styles. Our analysis shows that because different people have different language habits, ways of thinking and interests, this may lead to different users having different language styles. Intuitively, this difference in language style also affects the style of posts published by users. To investigate this phenomenon in more depth, we define the third question: \textbf{Do users' post titles have a personal style on social media? (Q3)} 


% 为了严谨的研究每个作者的标题是否具有个人风格，我们对比相同作者的标题对和不同作者的标题对之间文本相似度的区别。
In order to carefully investigate whether each author's title has a personal style, we compare the difference in text similarity between title pairs of the same author and between title pairs of different authors.
% 我们采样10万个标题对，这里的每个标题对里面的两个标题来自于同一作者，并计算这10万标题对的平均文本相似度。
We sample 100,000 title pairs, where two titles inside each title pair are from the same author, and calculate the averaged text similarity of these 100,000 title pairs.
% 相同，我们也会采样并计算标题来自于不同作者的10万个标题对的平均文本相似度。
Similarly, we also sample and calculate the averaged text similarity of 100,000 title pairs whose titles come from different authors.

% 这里和上文相同，我们是用words overlap作为衡量文本相似度的方法

% words overlap不光可以识别两段文本之间的语义重叠程度，而且可以直观的反映出 作者生成标题时 在排版格式上使用词语的重复。
The \textit{words overlap} not only identifies the degree of semantic overlap between two pieces of text, but also directly reflects the repetition of words used in the typesetting format when the author generates these titles.

% 展示图表，进行分析
% 同一个作者的不同标题之间可能有语义上的相似，和一些常用词的相似
% 根据图1a，我们可以清晰地发现来自相同作者的标题对的平均文本相似度远高于不同作者的。
As shown in Fig.~todo, we can clearly find that the average text similarity of title pairs from the same author is much higher than that of different authors.
% 具体分析，举几个例子 todo
% 通过控制是否采样同一作者的标题对，我们可以得到结论 用户的标题具有明确的个人风格：用户会根据自己的喜好和习惯对标题进行创作。
By controlling whether to sample the same author's title pairs, we can conclude that \textbf{users' titles have a clear personal style}: users create titles according to their preferences and habits.

% ----------Question four----------
% 2.标题不光可以作为识别文章主题的一段文本，受众同时可以通过标题的排版风格和用词风格来识别这篇文章的作者。
% 无论是在应用的外部缩略图还是文章的展示画面，标题都是首先映入眼帘的一段文本。直觉上，文本向受众传达这篇文章的主题和内容，受众在外部视图根据
% ----- ----- ----- -----
In the analysis of \secref{Q1}, we learned that the more the headline is in line with the current trend, the more it will attract the audience's attention and increase the popularity of the post. Intuitively, audiences do not only like to see posts about popular topics; they may also like posts about celebrities or acquaintances. The headline acts as the first thing the audience can see. Audiences may instinctively distinguish users by the different typographic and wording styles in headlines. So users with a distinct personal style are more likely to be identified by the audience and thus attract more of the audience's attention. To study more closely the relationship between personal style and popularity, the fourth question is: \textbf{What is the influence of personal style on the popularity of a post? (Q4)}


To investigate this question, we introduce the \textit{Personal Style Index} ($PSI \in [0,1]$), which is an indicator of the degree of personal style in a user's headlines. Calculating $PSI$ with user $u$ is defined as:
\begin{equation}
    PSI_u = \frac{\sum_{h_i \in H_u} \sum_{h_j \in H_u} WO(h_i, h_j)}{{(\#(H_u))^2}},
\end{equation}
where $H_u$ denotes the latest 20 post headlines of user $u$. The higher the $PSI$, the more obvious the personal style of the user's post headlines. When $PSI$ is equal to $1$, it means that the latest 20 post headlines of this user are exactly the same.
To observe the relationship between popularity and personal style, we use the average number of likes (aka thumbs-up) of a user's latest 20 posts to indicate the popularity of the user's posts.
Calculating the popularity of user $u$'s posts ($popularity_u \in \mathbb{Q}+$) is defined as:
\begin{equation}
    popularity_u = \frac{\sum_{p_i \in P_u} log(likes(p_i))}{{\#(P_u)}},
\end{equation}
where $P_u$ denotes the latest 20 post of user $u$, $likes()$ denotes the number of likes of the corresponding post and $log()$ is the logarithmic operator.
For easier observation, we group users by the $PSI$, and compare their average $popularity$ in the 5 intervals of $PSI$, as illustrated in Fig.~todo.
% 先展示一下结果
% 然后分析
AL vs. PSI
As shown in Fig.~, 
% 两个结论
% 在想象中，我们会更在意文章的内容。但其实我们有的时候会更在意这个文章是谁发的，这个时候，个人风格就有作用。



